Queue-Learning: A Reinforcement Learning Approach for Providing Quality of Service

End-to-end delay is a critical attribute of quality of service (QoS) in application domains such as cloud computing and computer networks. This metric is particularly important in tandem service systems, where the end-to-end service is provided through a chain of services. Service-rate control is a common mechanism for providing QoS guarantees in service systems. In this paper, we introduce a reinforcement learning-based (RL-based) service-rate controller that provides probabilistic upper-bounds on the end-to-end delay of the system, while preventing the overuse of service resources. In order to have a general framework, we use queueing theory to model the service systems. However, we adopt an RL-based approach to avoid the limitations of queueing-theoretic methods. In particular, we use Deep Deterministic Policy Gradient (DDPG) to learn the service rates (action) as a function of the queue lengths (state) in tandem service systems. In contrast to existing RL-based methods that quantify their performance by the achieved overall reward, which could be hard to interpret or even misleading, our proposed controller provides explicit probabilistic guarantees on the end-to-end delay of the system. The evaluations are presented for a tandem queueing system with non-exponential inter-arrival and service times, the results of which validate our controller's capability in meeting QoS constraints.

==> RL_implement.tex <==
\section{Implementation}

==> RLintro.tex <==
\section{Background on Reinforcement Learning}\label{RLintro}

% In this section, we briefly review the basic concepts of the reinforcement learning and discuss the average-reward setting.
% The basic elements of a reinforcement learning problem are the \emph{agent} and the \emph{environment}, which have iterative interactions with each other. The environment is modeled by a Markov decision process (MDP), which is specified by $<\mathcal{S},\mathcal{A},\mathcal{P},\mathcal{R}>$, with state space $\mathcal{S}$, action space $\mathcal{A}$, state transition probability matrix $\mathcal{P}$ and reward function $\mathcal{R}$. At each time step $t$, the agent observes a state $s_t \in \mathcal{S}$, takes action $a_t \in \mathcal{A}$, transits to state $s_{t+1} \in \mathcal{S}$ and receives a reward of $\mathcal{R}(s_t,a_t,s_{t+1})$. The agent's actions are defined by its policy $\pi$, where $\pi(a|s)$ is the  probability of taking action $a$ in state~$s$.

% The formal definition of an agent's goal varies based on the problem setting. In episodic tasks in which there is a notion of terminal state, the goal of the agent is to maximize the long-term expected \emph{return}, where the return is defined as $G_t = \sum_{k=t+1}^T R_k
% $. In continuing settings, in which the interaction between the agent and the environment continues forever, we cannot use the same return function as before, since $T=\infty$ and the reward can easily become unbounded. One way of handling this issue is by using \emph{discounting}. In this approach, the agent tries to maximize the expected discounted return, which is defined as $G_t = \sum_{k=t+1}^T \gamma^{k-t-1} R_k$, $0\leq \gamma<1$. In the discounted setting, the agent cares more about the immediate rewards in the near future rather than the delayed rewards in the far future. However, in many applications such as computer networks, we are interested in the average performance of the system in the long run and we care as much about the future as we do about the present. There is a third setting for formulating the goal in RL problems, which is called the \emph{average reward} setting\cite{sutton}. In this setting, the goal of the agent is to maximize the average reward per time step, which under \emph{ergodicity} assumption can be obtained as
% \begin{equation}
%     r(\pi) = \sum_s p_{\pi}^s(s) \sum_a \pi(a|s) \sum_{s',r} P(s',r|s,a)r,
% \end{equation}
% where $p_{\pi}^s(s)$ is the steady state distribution of being in state $s$ in a given time step following policy $\pi$. The average reward setting is a good candidate for formulating the goal in continuing environments, where we care about the future as much as the present. The \emph{differential} return is defined as $G_t = \sum_{k=t+1}^\infty (R_k-r(\pi))$. Similar to the notion of action-value function in the discounted setting, we can define differential action-value function (Q-function) as  $Q_\pi(s,a)=\mathbb{E}_\pi[G_t|s_t=s,a_t=a]$, which denotes the expected return starting from state $s$, taking action $a$, and following policy $\pi$. Defining the optimal Q-function as $Q^*(s,a)=\max_{\pi}Q_{\pi}(s,a)$, we can obtain the optimal policy as
% \begin{equation}
% \pi^*(a|s) = \left\{
% \begin{array}{ll}
% 1\qquad \text{if} & a={\arg \max}_{a'} Q^*(s,a'),\\
% 0\qquad & \text{otherwise}.
% \end{array} \right.
% \end{equation}
% The optimal Q-function must satisfy the Bellman optimality equation for the average reward setting as follows 
% \begin{equation}
%     Q^*(s,a)=\mathbb{E}_\pi\bigg[r-\max_\pi r(\pi)+\max_{a'} Q^*(s',a')\Big|s,a\bigg].
% \end{equation}
% Similar to the discounted setting, the Bellman optimality equation is not usually directly used to obtain the optimal Q-function. Instead, we use an iterative method to solve the Bellman equation, which is similar to the well-known Q-learning algorithm and is called \emph{R-learning}~\cite{rlearning}. Based on this method, the Q-function is updated at each time step as
% % {\small
% \begin{equation}
%     Q(s_t,a_t)\hspace{-0.1cm}\leftarrow \hspace{-0.1cm} Q(s_t,a_t)+\alpha \hspace{-0.06cm} \big[r_{t+1}-\bar{r}+\max_a Q(s_{t+1},a)-Q(s_t,a_t\hspace{-0.06cm})\big]\hspace{-0.08cm},
% \end{equation}
% % }
% where $\alpha$ represents the learning rate and $\bar{r}$ is an approximation of $r(\pi)$. At each time step that the behaviour policy acts greedily, i.e., $a_t=\arg\max_a Q(s_t,a)$, $\bar{r}$ is updated as
% \begin{equation}
%     \bar{r}\leftarrow \bar{r}+\beta \big[r_{t+1}-\bar{r}+\max_a Q(s_{t+1},a)-Q(s_t,a_t)\big],
% \end{equation}
% where $\beta$ is the step-size parameter.
